TTAQ: Towards Stable Post-training Quantization in Continuous Domain Adaptation

Post-training quantization (PTQ) reduces excessive hardware cost by quantizing full-precision models into lower bit representations on a tiny calibration set, without retraining. Despite the remarkable progress made through recent efforts, traditional PTQ methods typically encounter failure in dynamic and ever-changing real-world scenarios, involving unpredictable data streams and continual domain shifts, which poses greater challenges. In this paper, we propose a novel and stable quantization process for test-time adaptation (TTA), dubbed TTAQ, to address the performance degradation of traditional PTQ in dynamically evolving test domains. To tackle domain shifts in quantizer, TTAQ proposes the Perturbation Error Mitigation (PEM) and Perturbation Consistency Reconstruction (PCR). Specifically, PEM analyzes the error propagation and devises a weight regularization scheme to mitigate the impact of input perturbations. On the other hand, PCR introduces consistency learning to ensure that quantized models provide stable predictions for same sample. Furthermore, we introduce Adaptive Balanced Loss (ABL) to adjust the logits by taking advantage of the frequency and complexity of the class, which can effectively address the class imbalance caused by unpredictable data streams during optimization. Extensive experiments are conducted on multiple datasets with generic TTA methods, proving that TTAQ can outperform existing baselines and encouragingly improve the accuracy of low bit PTQ models in continually changing test domains. For instance, TTAQ decreases the mean error of 2-bit models on ImageNet-C dataset by an impressive 10.1\%.

==> tables/alg.tex <==
\vspace{0.2in}
\begin{algorithm}[h]
\small
\caption{Pipeline of TTAQ framework.} 
\label{alg:flow} 
\begin{algorithmic}[1]
\STATE {\color[rgb]{1,0,0}\# Post-Training Quantization stage:}
\STATE \textbf{Input:} Pre-trained model $\mathcal{M}$ and calibration set $\mathcal{C}$
\STATE \textbf{Output:} Optimal scale $s$, zero point $z$, quantized model $\mathcal{M}^q$
\STATE \# Calibration with PEM
\FOR{each sample $c \in \mathcal{C}$}
\STATE Apply the weight quantizer based on \equref{reg} ;\\
\STATE Initialize the scale $s$ and zero point $z$ based on \equref{sz};\\
\ENDFOR
\STATE \# Calibration with PCR
\FOR{each b $c \in$ Block $\mathcal{B}$}
\FOR{$i \in \textit{iters}$}
\STATE Compute reconstruction loss $\mathcal{L}_{recon}$ based on \equref{reconstruction} ;\\
\STATE Compute perturbation consistency loss $\mathcal{L}_{prcl}$ with \equref{pcrl};\\
\STATE Backward propagate $\mathcal{L}_{recon}$ and $\mathcal{L}_{prcl}$;\\
\STATE Update the optimizer ;\\
\ENDFOR
\ENDFOR
\RETURN scale $s$, zero point $z$, and quantized model $\mathcal{M}^q$;


\STATE {\color[rgb]{1,0,0}\# Continual Test-Time Adaption stage:}
\STATE \textbf{Input:} Quantized model $\mathcal{M}^q$ and Streaming data $\mathcal{X}$
\STATE \textbf{Output:} Prediction $\mathcal{Y}$
\STATE Initialize and Freeze Source Model $f\left(x; \Theta_0\right)$ and test-time model $f\left(x; \Theta_t\right)$  with $\mathcal{M}^q$.
\STATE Initialize class-wise factor $\pi_0$.
\STATE Set weights and biases of BN layers in $f\left(x; \Theta_t\right)$ to be trainable.

\FOR{$t \in$ time $\textit{T}$}
\STATE Data augmentation ;\\
\STATE Compute adaptive balanced loss $\mathcal{L}_{abl}$ based on \equref{abl};\\
\STATE Backward propagation $\mathcal{L}_{abl}$;\\
\STATE Compute class importance factor $\pi_t$ based on \equref{pi};
\STATE Update the optimizer;\\
\RETURN prediction $\mathcal{Y}_t$;
\ENDFOR


\end{algorithmic}
\end{algorithm}



==> tables/deit.tex <==
\begin{table*}[!h]
\renewcommand{\arraystretch}{1.2}
\centering
\small
\caption{Classification error rate~(\%) for the Quantized Deit-S on ImageNet-C dataset.}% For CIFAR100C the results are evaluated on ResNeXt (W2A4), for CIFAR10C on WideResNet (W2A4).} 
\label{tab:deit}
\scalebox{0.74}{
\tabcolsep=4pt
\begin{tabular}{l|l|ccccccccccccccc|c}\toprule
& \multicolumn{1}{l|}{Time} & \multicolumn{15}{l|}{$t\xrightarrow{\hspace*{14.5cm}}$}& \\ \hline
\rotatebox[origin=c]{90}{\#Bits}& Method & \rotatebox[origin=c]{70}{Gaussian} & \rotatebox[origin=c]{70}{Shot} & \rotatebox[origin=c]{70}{Impulse} & \rotatebox[origin=c]{70}{Defocus} & \rotatebox[origin=c]{70}{Glass} & \rotatebox[origin=c]{70}{motion} & \rotatebox[origin=c]{70}{Zoom} & \rotatebox[origin=c]{70}{Snow} & \rotatebox[origin=c]{70}{Frost} & \rotatebox[origin=c]{70}{Fog}  & \rotatebox[origin=c]{70}{Brightness} & \rotatebox[origin=c]{70}{Contrast} & \rotatebox[origin=c]{70}{Elastic} & \rotatebox[origin=c]{70}{Pixelate} & \rotatebox[origin=c]{70}{Jpeg} & Mean \\
\midrule
& Full precision & 58.66 & 50.98 & 51.28 & 61.12 &56.20 & 49.18 &51.78 &43.96 &42.04 & 39.86 & 27.04 &50.66 & 45.92 & 44.92 & 39.32 & 50.30
\\
\midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{W4A6}}
% \cline{2-18}
& Adaround  &76.18 &68.12 &67.42 &73.96 &67.04 &62.50 &59.94 &59.52 &52.94 &47.52 &35.88 &71.78 &56.06 &56.48 &48.54 & 60.24 \\
& Brecq      &65.74 & 58.24 & 56.76 & 65.20 & 58.42 & 53.14 & 54.50 & 48.62 & 45.74 & 40.48 & 29.40 & 56.70 & 49.44 & 48.62 & 41.80 & 51.47\\
& QDrop &64.94 & 57.88 & 56.72 & 65.56 & 60.14 & 53.20 & 55.40 & 49.38 & 45.92 & 40.82 & 29.58 & 59.16 & 50.94 & 49.72 & 42.84 & 52.15\\
& TTAQ (ours)   &\textbf{63.60} & \textbf{55.98} & \textbf{54.66} & \textbf{63.98} & \textbf{57.46} & \textbf{52.34} & \textbf{52.94} & \textbf{45.76} & \textbf{43.64} & \textbf{39.66} & \textbf{27.86} & \textbf{54.72} & \textbf{49.34} & \textbf{47.70} & \textbf{41.32} & \underline{\textbf{50.06}}\\
\midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{W2A6}}
% \cline{2-18}
& Adaround  &99.36 & 99.14 & 99.60 & 96.98 & 96.14 & 95.84 & 94.30 & 96.98 & 95.08 & 95.38 & 84.70 & 99.58 & 94.06 & 97.24 & 92.36 & 95.76 \\
& Brecq      &97.90 & 99.62 & 99.84 & 86.10 & 74.88 & 70.62 & 66.98 & 74.40 & 64.06 & 58.84 & 43.16 & 81.78 & 64.58 & 68.06 & 58.58 & 73.98\\
& QDrop &92.40 & 86.28 & 83.88 & 81.24 & 75.54 & 73.22 & 68.00 & 75.50 & 64.02 & 60.54 & 43.28 & 93.94 & 66.06 & 67.98 & 59.88 & 72.78\\
& TTAQ (ours)   &\textbf{85.86} & \textbf{76.10} & \textbf{76.50} & \textbf{77.52} & \textbf{70.24} & \textbf{65.28} & \textbf{65.20} & \textbf{66.98} & \textbf{61.76} & \textbf{54.06} & \textbf{40.06} & \textbf{79.36} &\textbf{ 60.88} & \textbf{62.42} & \textbf{54.56 }& \underline{\textbf{66.45}}\\
\bottomrule
\end{tabular}
}
\label{tab:cifar}
\end{table*}
